Can semi-supervised learning use all the data effectively? A lower bound perspective

Prior works have shown that semi-supervised learning algorithms can leverage unlabeled data to improve over the labeled sample complexity of supervised learning (SL) algorithms. However, existing theoretical analyses focus on regimes where the unlabeled data is sufficient to learn a good decision boundary using unsupervised learning (UL) alone. This begs the question: Can SSL algorithms simultaneously improve upon both UL and SL? To this end, we derive a tight lower bound for 2-Gaussian mixture models that explicitly depends on the labeled and the unlabeled dataset size as well as the signal-to-noise ratio of the mixture distribution. Surprisingly, our result implies that no SSL algorithm can improve upon the minimax-optimal statistical error rates of SL or UL algorithms for these distributions. Nevertheless, we show empirically on real-world data that SSL algorithms can still outperform UL and SL methods. Therefore, our work suggests that, while proving performance gains for SSL algorithms is possible, it requires careful tracking of constants.

==> extra.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[Tight Excess Risk Lower Bound]

There exist constants $C_0, C_1 > 0$ such that for any $\snr>0$, for any sufficiently large $\nunl$, $\nlab$ and $d$, we have
\begin{equation}
    \inf_{\algssl} \sup _{\left\|\theta_*\right\|=\snr} \EE_{\Dlab \sim
    \left(\jointsnr\right)^{\nlab}, \Dunl \sim
  \left(\marginalsnr\right)^{\nunl}} \errssl \geq C_0 e^{-\snr^2/2} \min \left\{  \frac{d}{\snr \nlab + \snr^3 \nunl} , s\right\}
\end{equation}
Furthermore, there exists an algorithm whose excess risk can be upper bounded
like $$\EE_{\Dlab \sim
    \left(\jointsnr\right)^{\nlab}, \Dunl \sim
  \left(\marginalsnr\right)^{\nunl}} \errssl \leq \Tilde{C_0}e^{-\snr^2/2} \min \left\{  \frac{d}{\snr \nlab} ,  \frac{d}{\snr^3 \nunl}+e^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2} \right\} $$ for large enough $\nlab$ or $\nunl$ where $\snr = \| \thetastar \|$. 
\end{theorem}


\begin{theorem}[Parameter Estimation Lower Bound]
There exist universal constants $C_0, C_1 \geq 0$ such that, for any $d\geq2$,
$\nunl \geq d$ and $0 \leq \snr \leq 1$, we have 

\begin{equation*}
    \inf _{\hat{\theta}} \sup _{\left\|\theta_*\right\|=\snr} \EE_{\Dlab \sim
    \left(\jointsnr\right)^{\nlab}, \Dunl \sim
  \left(\marginalsnr\right)^{\nunl}} \estimerr(\algssl, \Dlab, \Dunl) \geq  C_0
  \min \left\{ s, \sqrt{\frac{d}{C_1 \nlab+ \snr^2 \nunl}} \right\}.
\end{equation*}
Furthermore, there exists an algorithm whose upper bound on the estimation error
matches the rates of the lower bound: $\EE_{\Dlab \sim
    \left(\jointsnr\right)^{\nlab}, \Dunl \sim
  \left(\marginalsnr\right)^{\nunl}} \estimerr(\algssl, \Dlab, \Dunl) 
 \leq C' \min \left\{ s, \sqrt{\frac{d}{\nlab}}, \sqrt{\frac{d}{ \snr^2 \nunl} + se^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2} } \right\}$, where
  $\snr=\|\thetastar\|$.
\end{theorem}


\begin{theorem}[Tight Excess Risk Lower Bound]
For any $\snr \in [0, 1]$, for any sufficiently large $d$, we have
\begin{equation}
  \inf_{\algssl} \sup _{\left\|\theta_*\right\|=\snr} \EE\bs{ \errssl} \gtrsim e^{-\snr^2/2} \min \left\{
\frac{d}{\snr \nlab + \snr^3 \nunl} , s\right\},
\end{equation}
where the expectation is over $\Dlab \sim
    \left(\jointsnr\right)^{\nlab}$ and $\Dunl \sim
  \left(\marginalsnr\right)^{\nunl}$. Furthermore, for any sufficiently large $\nlab$ and $\nunl$, there exists an algorithm whose excess risk can be upper bounded
  like $$\EE \bs{\errssl} \lesssim e^{-\snr^2/2} \min \left\{  \frac{d}{\snr \nlab} ,  \frac{d}{\snr^3 \nunl}+e^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2} \right\} $$, where $\snr = \| \thetastar \|$. 
\end{theorem}

\begin{theorem}[Minimax Rates for Parameter Estimation]
For any $d\geq2$,
$\nunl \geq d$ and $0 \leq \snr \leq 1$, we have 
\begin{equation*}
    \inf _{\hat{\theta}} \sup _{\left\|\theta_*\right\|=\snr} \EE\bs{\estimerr(\algssl, \Dlab, \Dunl)} \gtrsim
  \min \left\{ s, \sqrt{\frac{d}{C_1 \nlab+ \snr^2 \nunl}} \right\},
\end{equation*}
where the expectation is over $\Dlab \sim
    \left(\jointsnr\right)^{\nlab}$ and $\Dunl \sim
  \left(\marginalsnr\right)^{\nunl}$. Furthermore, for sufficiently large $\nlab$ or $\nunl$ there exists an algorithm whose upper bound on the estimation error
matches the rates of the lower bound: $\EE \bs{\estimerr(\algssl, \Dlab,
\Dunl)}
 \lesssim \min \left\{ s, \sqrt{\frac{d}{\nlab}}, \sqrt{\frac{d}{ \snr^2 \nunl} + se^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2} } \right\}$, where
  $\snr=\|\thetastar\|$.
\end{theorem}

\begin{restatable}{theorem}{thmparamestsslupper}[Parameter Estimation Upper bound]  \label{thm:param_est_upper}
    Let $\hat{\theta}_{SSL} = t^* \hat{\theta}_{SL} + (1-t^*) \hat{\theta}_{UL}$ where $t^*$ is as given in Lemma \ref{lem:combine} with the supervised estimator $\hat{\theta}_{SL} = \frac{1}{\nlab} \sum_{i=1}^{\nlab} Y_i X_i$ and the unsupervised estimator $\hat{\theta}_{UL} = \hat{\snr}\hat{v}$ with $\hat{\snr} = \sqrt{(\hat{\lambda}-1)_+}$, where $\hat{\lambda}$ is the leading eigenvalue of the sample covariance matrix $\hat{\Sigma} = \frac{1}{\nunl} \sum_{j=0}^{\nunl} \Tilde{X_j} \Tilde{X_j} ^T$ and $\hat{v}$ is the corresponding eigenvector. Then for all $\thetastar$ such that $\nrm{\thetastar} = \snr$,
    
    \begin{equation}
        \mathbb{E} \nrm{\hat{\theta}_{SSL} - \thetastar} \leq \Tilde{C_0} \sqrt{\frac{d}{\Tilde{C_l} \nlab+ \snr^2 \nunl}} 
    \end{equation}
    \end{restatable}

\begin{proof}
    Using Jensen's, Lemma \ref{lem:combine} and the upperbounds for the relative stimators we have
    \begin{align}
    \EE \nrm{\thetahat_{SSL} - \thetastar} &\leq  \sqrt{\EE \nrm{\thetahat_{SSL} - \thetastar} ^2 }  \notag \\
    &= \sqrt{\frac{1}{\frac{1}{\EE [ \nrm{\thetahat_{SL} - \thetastar}^2]}+\frac{1}{\EE [ \nrm{\thetahat_{UL} - \thetastar}^2]}}  } \notag \\
    & \leq \sqrt{ \frac{1}{\frac{\nlab}{d}+\frac{s^2 \nunl}{C'' d}} }  \notag \\
    &= \tilde{C_0} \sqrt{ \frac{d}{\Tilde{C_l}\nlab + s^2 \nunl} } \notag 
\end{align}
\end{proof}

For the unsupervised estimator we consider $\thetahat_{UL} = \hat{\snr}\hat{v}$ with $\hat{\snr} = \sqrt{(\hat{\lambda}-1)_+}$, where $\hat{\lambda}$ is the leading eigenvalue of the sample covariance matrix $\hat{\Sigma} = \frac{1}{\nunl} \sum_{j=0}^{\nunl} \Tilde{X_j} \Tilde{X_j} ^T$ and $\hat{v}$ is the corresponding eigenvector. 

We have now all the elements to prove Theorem \ref{thm:param_est_upper}

%\thmparamestsslupper*

\begin{proposition}[Fixing the sign of $\thetaul$]\label{prop:ul+}
%     Let $\thetahat_{SL} =  \frac{1}{\nlab} \sum_{i=1}^{\nlab} Y_i X_i $ and $\hat{\theta}_{UL} = \hat{\snr}\hat{v}$ with $\hat{\snr} = \sqrt{(\hat{\lambda}-1)_+}$, where $\hat{\lambda}$ is the leading eigenvalue of the sample covariance matrix $\hat{\Sigma} = \frac{1}{\nunl} \sum_{j=0}^{\nunl} \Tilde{X_j} \Tilde{X_j} ^T$ and $\hat{v}$ is the corresponding eigenvector. Consider the following estimator that fixes the permutation of the unsupervised estimator:
%     \begin{equation}
%         \thetahat_{UL+} = \sign\left(\thetahat_{SL}^\top  \thetahat_{UL}\right)  \thetahat_{UL}. \notag
%     \end{equation}
  Consider the UL+ estimator $\thetaulp$ defined in Equation~\ref{eq:ulplus}.
    There exist universal constants $C, C'>0$ such that for $\nunl \geq (160/s)^2 d$
    \at{change so that it doesn't have square estimation error; no need for it
    anymore}
    \at{change the proof as well}
    \begin{align}
     \EE \left[  \nrm{\thetahat_{UL+} - \thetastar}^2 \right] &\leq C \frac{d}{s^2 \nunl} + C' s  e^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2}. \notag
    \end{align}
\end{proposition}

\begin{proof}
    Let $
    \thetahat_{UL+} = \sign\left(\thetahat_{SL}^\top  \thetahat_{UL}\right)  \thetahat_{UL} =: \sgnhat \thetahat_{UL}.$

And denote $\sgn = \sign ({{\thetastar}^\top \thetahat_{UL} }) = \argmin_{\Tilde{\sgn}\in \{-1, +1\}} \nrm{\Tilde{\sgn} \thetahat_{UL} - \thetastar}^2  $

Note that we can write the expected squared estimation error of $ \thetahat_{UL+}$ as:
\begin{align}
    \EE \left[  \nrm{\thetahat_{UL+} - \thetastar}^2 \right] &=  \EE \left[  \nrm{\sgnhat \thetahat_{UL} - \thetastar}^2 \right] \notag \\
    &=  \EE \left[  \indicator{\sgnhat = \sgn} \nrm{\sgn \thetahat_{UL} - \thetastar}^2 + \indicator{\sgnhat \neq \sgn} \nrm{\sgn \thetahat_{UL} + \thetastar}^2 \right] \notag \\
    &=  \EE \left[  \indicator{\sgnhat = \sgn} \nrm{\sgn \thetahat_{UL} - \thetastar}^2 + \indicator{\sgnhat \neq \sgn} \nrm{\sgn \thetahat_{UL} -\thetastar + 2\thetastar}^2 \right] \notag\\
    &\leq  \EE \left[  \indicator{\sgnhat = \sgn} \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right] \notag \\
    & \hspace{30pt}+ \EE \left[ \indicator{\sgnhat \neq \sgn} ( \nrm{\sgn \thetahat_{UL} -\thetastar }^2+ 4\nrm{\thetastar}^2 + 4 \nrm{\thetastar} \nrm{\sgn \thetahat_{UL} - \thetastar}  ) \right] \notag \\
    &= \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right] + \EE \left[  \indicator{\sgnhat \neq \sgn} ( 4\snr^2 + 4 \snr \nrm{\sgn \thetahat_{UL} - \thetastar}  ) \right] \notag \\
    &\leq \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right] + 4 \snr^2 \prob{(\sgnhat \neq \sgn)} \notag\\
    &\hspace{30pt}+  4 \snr \sqrt{\EE \left[  \indicator{\sgnhat \neq \sgn} \right] \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2  \right] } \notag \\
    &= \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right] + 4 \snr^2 \prob{(\sgnhat \neq \sgn)} \notag \\
    &\hspace{30pt} +4 \snr \sqrt{\prob{(\sgnhat \neq \sgn)} \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2  \right] } \notag \\
    &\leq \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right] + 4 \snr^2 \prob{(\sgnhat \neq \sgn)} \notag \\
    &\hspace{30pt}+  2 \snr \left(  {\prob{(\sgnhat \neq \sgn)} + \EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2  \right] } \right)\notag \\
    &\leq \left( 1+2s \right)\EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right] + \left( 4 \snr^2 + 2\snr \right)\prob{(\sgnhat \neq \sgn)}. \label{eq:ulpluserrdecomposition}
\end{align}

Note that for the $\EE \left[  \nrm{\sgn \thetahat_{UL} - \thetastar}^2 \right]$ term we already have an upper bound from Proposition \ref{prop:ul}. Moreover, the probability of estimating the sign(permutation) wrong can be written as 

\begin{align}
    \prob{(\sgnhat \neq \sgn)} &= \prob{\left (Z \geq \sqrt{\nlab s^2 } \frac{|\thetahat_{UL}^\top \thetastar|}{\nrm{\thetahat_{UL}} \nrm{\thetastar}}\right)} \hspace{20pt} \text{where $Z\sim\mathcal{N}(0,1)$} \notag \\
    & \leq \prob(Z\geq \sqrt{\nlab s^2 } (1-A)) + \prob{\left (  \frac{|\thetahat_{UL}^\top \thetastar|}{\nrm{\thetahat_{UL}} \nrm{\thetastar}} \leq 1 - A \right)} \notag \\
    & \leq e^{-\frac{1}{2} \nlab \snr^2 (1-A)^2} + \prob{\left (  \frac{|\thetahat_{UL}^\top \thetastar|}{\nrm{\thetahat_{UL}} \nrm{\thetastar}} \leq 1 - A \right)}. \notag
\end{align}

Where we used the Chernoff bound in the last step. Now set $ A = c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}}$. Using Proposition 6 in \cite{NIPS2013_456ac9b0} for large enough $\nunl$ we have 

\begin{align}
    \prob{(\sgnhat \neq \sgn)} &\leq e^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2} + \frac{d}{\nunl}. \notag
\end{align}

Combining this with Equation \ref{eq:ulpluserrdecomposition} we get: 

\begin{align}
     \EE \left[  \nrm{\thetahat_{UL+} - \thetastar}^2 \right] &\leq C \frac{d}{s^2 \nunl} + C' s  e^{-\frac{1}{2} \nlab \snr^2 (1- c_0 \sqrt{\frac{d \log(\nunl)}{\snr^2 \nunl}})^2}. \notag
\end{align}
\end{proof}
